Increasing Interpretability of Neural Networks By Approximating Human Visual Saliency

Understanding specifically where a model focuses on within an image is critical for human interpretability of the decision-making process. Deep learning-based solutions are prone to learning coincidental correlations in training datasets, causing over-fitting and reducing the explainability. Recent advances have shown that guiding models to human-defined regions of saliency within individual images significantly increases performance and interpretability. Human-guided models also exhibit greater generalization capabilities, as coincidental dataset features are avoided. Results show that models trained with saliency incorporation display an increase in interpretability of up to 30% over models trained without saliency information. The collection of this saliency information, however, can be costly, laborious and in some cases infeasible. To address this limitation, we propose a combination strategy of saliency incorporation and active learning to reduce the human annotation data required by 80% while maintaining the interpretability and performance increase from human saliency. Extensive experimentation outlines the effectiveness of the proposed approach across five public datasets and six active learning criteria.

==> Figures/TeX/results_acc.tex <==

\begin{figure*}[t]
    \begin{subfigure}[b]{1\textwidth}
      \begin{subfigure}[b]{0.327\textwidth}
          \centering
            \includegraphics[width=1\textwidth]{Figures/Accuracy/cub_resnet_acc.png}
            \caption{CUB}
      \end{subfigure}
      \hfill
      \begin{subfigure}[b]{0.327\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{Figures/Accuracy/flowers_resnet_acc.png}
          \caption{Flowers}
      \end{subfigure}
      \hfill
      \begin{subfigure}[b]{0.327\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{Figures/Accuracy/imagenet_resnet_acc.png}
          \caption{ImageNet}
      \end{subfigure}
  \end{subfigure} \vskip3mm
  \centering
  \begin{subfigure}[b]{1\textwidth}
  \centering
      \begin{subfigure}[b]{0.327\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{Figures/Accuracy/skin_resnet_acc.png}
          \caption{Skin}
      \end{subfigure}
      % \hfill
      \begin{subfigure}[b]{0.327\textwidth}
          \centering
          \includegraphics[width=1\textwidth]{Figures/Accuracy/food_resnet_acc.png}
          \caption{Food}
      \end{subfigure}
   
  \end{subfigure} \vskip3mm
  \caption{CAPTION}
  \label{fig:test_accuracy}
  % \null\vskip-5mm
\end{figure*}

